On the Local Minima of the Empirical Risk

Population risk is always of primary interest in machine learning; however, learning algorithms only have access to the empirical risk. Even for applications with nonconvex nonsmooth losses (such as modern deep networks), the population risk is generally significantly more well-behaved from an optimization point of view than the empirical risk. In particular, sampling can create many spurious local minima. We consider a general framework which aims to optimize a smooth nonconvex function $F$ (population risk) given only access to an approximation $f$ (empirical risk) that is pointwise close to $F$ (i.e., $\|F-f\|_{\infty} \le \nu$). Our objective is to find the $\epsilon$-approximate local minima of the underlying function $F$ while avoiding the shallow local minima---arising because of the tolerance $\nu$---which exist only in $f$. We propose a simple algorithm based on stochastic gradient descent (SGD) on a smoothed version of $f$ that is guaranteed to achieve our goal as long as $\nu \le O(\epsilon^{1.5}/d)$. We also provide an almost matching lower bound showing that our algorithm achieves optimal error tolerance $\nu$ among all algorithms making a polynomial number of queries of $f$. As a concrete example, we show that our results can be directly used to give sample complexities for learning a ReLU unit.

==> abstract-old.tex <==
% !TeX root = main.tex 

Population risk---the expectation of the loss over the sampling mechanism---is 
always of primary interest in machine learning. However, learning algorithms only have access to empirical risk, which is the average loss over training examples. Although the two risks are typically guaranteed to be pointwise close, % through uniform convergence, 
for applications with nonconvex nonsmooth losses (such as modern deep networks), 
the effects of sampling can transform a well-behaved population risk into an 
empirical risk with a landscape that is problematic for optimization. 
The empirical risk can be nonsmooth, and it may have many additional local minima.

%While the population risk is always of primary interests in machine learning, the empirical risk --- typically guaranteed to be close to the population risk through uniform convergence --- is the one available to the training algorithms. For learning applications with nonconvex nonsmooth losses (such as modern deep networks), the effects of sampling can transform a well-behaved population risk into an empirical risk with bad landscape, typically nonsmooth, or even introducing many spurious local minima.

This paper considers a general optimization framework which aims to find approximate local minima of a smooth nonconvex function $F$ (population risk) given only access to the function value of another function $f$ (empirical risk), which is pointwise close to $F$ (i.e., $\norm{F-f}_{\infty} \le \nu$). We propose a simple algorithm based on stochastic gradient descent (SGD) on a smoothed version of $f$ which is guaranteed to find an $\epsilon$-second-order stationary point if $\nu \le O(\epsilon^{1.5}/d)$, thus escaping all saddle points of $F$ and all the additional local minima introduced by $f$. We also provide an almost matching lower bound  showing that our SGD-based approach achieves the optimal trade-off between $\nu$ and $\epsilon$, as well as the optimal dependence on problem dimension $d$, among all algorithms making a polynomial number of queries.
As a concrete example, we show that our results can be directly used to give sample complexities for learning a ReLU unit, whose empirical risk is nonsmooth.


==> conclusion.tex <==
% !TeX root = main.tex 


\section{Conclusion}

In this paper we design an optimization algorithm that can find a second-order stationary point of a nonconvex function, given only access to a perturbed version. In statistical learning, our algorithm can directly optimize the population risk, even though it only has access to the empirical risk, which may not have a well-behaved landscape. Our algorithm is accompanied by a matching lower bound that shows it achieves the optimal trade-off between error tolerance $\nu$, accuracy of solution $\epsilon$, and dimension $d$ among all polynomial-time algorithms. We also revealed a gap in error tolerance between the information-theoretic limit and what is solvable by algorithms making a polynomial number of queries, by providing upper and lower bounds for all (potentially exponential time) algorithms.

% In contrast to prior work \citep{zhang2017hitting}, the maximum function error tolerated by our algorithm has better dependence on optimization accuracy $\epsilon$ and dimension $d$, and we showed that this is optimal up to log factors by proving a matching lower bound for any polynomial query algorithms.
%We also revealed a gap between error tolerance between information theoretical limit and what is solvable by polynoimal queries algorithms, by providing upper and lower bounds for all (potentially exponential time) algorithms. Applications of this work are also discussed.

% For future work, we hope to ...


==> intro-old.tex <==
% !TeX root = main.tex 

\section{Introduction}

The optimization of nonconvex loss functions has been key to the success of 
modern machine learning.  While classical research in optimization focused
on convex functions that have a unique critical point that is both locally 
and globally minimal, a nonconvex function can have many local maxima, 
local minima and saddle points which pose significant challenges for 
optimization. A recent line of research has yielded significant progress
on one aspect of this problem---it has been established that favorable 
rates of convergence can be obtained even in the presence of saddle points, using 
simple variants of stochastic gradient descent~\citep[e.g.,][]{ge2015escaping, 
carmon16accelerated,agarwal17finding,jin17escape}.  These research results
have introduced new analysis tools for nonconvex optimization, and it is
of significant interest to begin to use these tools to attack the problems 
associated with undesirable local minima.

% While it is NP-hard to find global minima for a general nonconvex function, this paper shows how to efficiently avoid an important class of shallow local minima created by small perturbations to the ground truth function.
% %whose basins of attraction have ``low barriers'' 
% Suppose we are given a nonconvex function $f$ with a landscape that is problematic for optimization---possibly nonsmooth, with many `shallow' local minima---but we know that $f$ is close in function value to a well-behaved function $F$, which is smooth and do not have bad local minima, as shown in Figure \ref{fig:intro}a. Our objective is to find the `deep' local minima that persist in $F$, while avoiding those `shallow' local minima of $f$ that vanish in %the smoothed version %we shouldn't call F the smoothed version because later there is also f_\sigma and it can be confusing
% $F$.

It is NP-hard to avoid all of the local minima of a general nonconvex function. 
But there are some classes of local minima where we might expect that simple
procedures---such as stochastic gradient descent---may continue to prove effective.  
In particular, in this paper we consider local minima that are created by small 
perturbations to an underlying smooth objective function.  Such a setting is natural 
in statistical machine learning problems, where data arise from an underlying
population, and the population risk, $F$, is obtained as an expectation over
a continuous loss function and is hence smooth: $F(\btheta) = \E_{\z \sim \D}
[L(\btheta; \z)]$, for a loss function $L$ and population distribution $\D$.   
The sampling process turns this smooth risk into an empirical risk, 
$f(\btheta) = \sum_{i=1}^n L(\btheta; \z_i)/n$, which may be non-smooth and 
which generally will have many shallow local minima.  From an optimization 
point of view $f$ can be quite poorly behaved; indeed, it has been observed in 
deep learning that the empirical risk may have exponentially many shallow 
local minima, even when the underlying population risk is well-behaved and 
smooth almost everywhere \citep{brutzkus17globally,auer96exponentially}.
From a statistical point of view, however, we can make use of classical 
results in empirical process theory~\citep[see, e.g.,][]{boucheron,
bartlett03rademacher} to show that, under certain assumptions on the
sampling process, $f$ and $F$ are uniformly close:
\begin{equation}\label{eq:problem_intro}
    \norm{F - f}_{\infty} \le \nu. 
\end{equation}
See Figure \ref{fig:intro}(a) for a depiction of this result, and
Figure \ref{fig:intro}(b) for a depiction of the effect of sampling on
the optimization landscape.  We wish to exploit this nearness of $F$
and $f$, designing and analyzing optimization procedures that find the 
approximate local minima (see definition \ref{def:exactSOSP}) of the 
smooth function $F$, while avoiding those shallow minima that only exist in 
the sampled function $f$.

Although the relationship between population risk and empirical risk is
our major motivation, we note that other applications of our framework 
include two-stage robust optimization and private learning (see Section 
5.2). In these settings, $\eta$ can be viewed as the amount of adversarial 
perturbation or noise due to sources other than data sampling.  As in the
sampling setting, we hope to show that simple algorithms such as stochastic 
gradient descent are able to escape the shallow local minima that arise 
for relatively small values of $\eta$.

%This problem naturally arises in the context of \textit{empirical risk minimization (ERM)}, where $(f, F)$ are the empirical and population risks.
%Given a nonconvex loss function $L(\btheta; \z)$ and data $\z_i$ sampled from an underlying distribution $\D$, the population risk $F(\btheta) = \E_{\z \sim \D}[L(\btheta; \z)]$ is the expectation of the loss function over the distribution $\D$; the empirical risk $f(\btheta) = \sum_{i=1}^n L(\btheta; \z_i)/n$ is the average of loss function over $n$ samples. While population risk is of primary interest in machine learning, learning algorithms only have access to the empirical risk. The pointwise closeness between the two is typically guaranteed by uniform convergence results from classical empirical process theory \citep{boucheron,bartlett03rademacher}.  It is observed in deep learning that the empirical risk may have a landscape that is problematic for optimization, including exponentially many shallow local minima, even when the underlying population risk is well-behaved and smooth almost everywhere \citep{brutzkus17globally,auer96exponentially}, as illustrated in Figure \ref{fig:intro}b.


% The empirical risk is often known to have a landscape that is problematic for optimization, even when the underlying population risk is well-behaved, as illustrated in Figure \ref{fig:intro} b. For example,
% the empirical risk can be nonsmooth in an entire subspace while the population 
% risk is smooth except at a single point (e.g., for convolution networks with 
% Gaussian inputs \citep{brutzkus17globally}). Sampling can introduce 
% exponentially many local minima \citep{auer96exponentially}. 
% In the context of deep learning, many researchers turn to studying the 
% population risk \citep{brutzkus17globally, li2017convergence} while analysis
% of its finite-sample version remains elusive, making it difficult to rule out the existence of local minima. %Even in low-rank matrix problems where analysis of the population risk is straightforward, the analysis of the empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}. 
% This motivates optimization algorithms that are immune to `shallow' local minima.




% In some applications \cite[e.g.][]{bhoj16global, ge2016matrix}, all the local minima are desirable solutions, while saddle points are not acceptable. Recent results in nonconvex optimization \citep[e.g.,][]{ge2015escaping, carmon16accelerated,agarwal17finding,jin17escape} guarantee avoiding saddle points when the objective function is smooth.  In contrast, our understanding of undesirable local minima is very limited. Although such local minima have suboptimal loss, the aforementioned guarantees do not preclude convergence to such minima.
% % in practical learning problems, one often encounters functions that are nonsmooth and have undesirable local minima, in which case these guarantees are no longer applicable.
% %Two key obstables to this are saddle points and local minima with suboptimal loss. 

% Since one cannot hope to deal with arbitrarily bad local minima, this paper is concerned with resolving an important class of spurious local minima that arises naturally in nonconvex \textit{empirical risk minimization}. Suppose we want to minimize a nonconvex function $f$, which may have a landscape that is problematic for optimization--- nonsmooth, with many poor local minima. Further, suppose it is known that $f$ is close in function value to $F$, which is also nonconvex but smooth and has no poor local minima, even though their higher order derivatives may be far apart (see Figure \ref{fig:intro}a):
% \begin{equation*}
% 	\norm{F - f}_{\infty} \le \nu. 
% \end{equation*}
% We do not have access to $F$, but would like to use this property to avoid poor local minima in $f$. Specifically, we want to converge to a ``flat'' local minimum of $f$---one that is close to being a local minimum in the smooth function $F$---as opposed to a ``sharp'' local minimum of $f$, that is, one that is far from being a local minimum in $F$.

% Let us consider the motivating application, empirical risk minimization.  
% Given a nonconvex loss function $L(\btheta; \z)$ and data $\z_i$ sampled from 
% an underlying distribution $\D$, the population risk $\poploss$ and empirical 
% risk $\emploss$ are $	\poploss(\btheta) = \E_{\z \sim \D}[L(\btheta; \z)]$ and $ \emploss(\btheta) = \frac{1}{n}\sum_{i=1}^n L(\btheta; \z_i)$ respectively. Learning algorithms only have access to the empirical risk---the average loss over training examples. Yet the empirical risk is often known to have a landscape that is problematic for optimization, even when 
% the underlying population risk is well-behaved, as illustrated in Figure \ref{fig:intro}.  Indeed,
% the empirical risk can be nonsmooth in an entire subspace while the population 
% risk is smooth except at a single point (e.g., for convolution networks with 
% Gaussian inputs \citep{brutzkus17globally}), and sampling can introduce 
% exponentially many spurious local minima \citep{auer96exponentially}. 
% In the context of deep learning, many researchers turn to studying the 
% population risk \citep{brutzkus17globally, li2017convergence} while analysis
% of its finite-sample version remains elusive, making it difficult to rule out the existence of poor local minima. Even in low-rank matrix problems 
% where analysis of the population risk is straightforward, the analysis of the 
% empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}. 


%\cnote{Put empirical risk after formulation, shorten current two paragraph, suffice to argue why our formulation is natual and interesting.}


\begin{figure}[t]
	\centering
	\includegraphics[width=0.28\textwidth, trim=80 70 250 10, clip]{nu_example.pdf}%
	\includegraphics[width=0.36\textwidth, trim=0 30 30 10, clip]{intro_pop}%
	\includegraphics[width=0.36\textwidth, trim=0 30 30 10, clip]{intro_emp}
	\caption{a) Function error $\nu$; b) Population risk vs empirical risk} \label{fig:intro}
\end{figure}
%\cnote{make f and F color in Figure 1 more distinguishable?}

% Fortunately, the empirical risk is typically pointwise close to the population risk and in some cases, one can show that the population risk is smooth and has no spurious local minima  \citep{brutzkus17globally, li2017convergence}. Using our formulation from earlier, $(F, f)$ might be the population and 
% empirical risk, $(\poploss, \emploss)$.  The function error $\nu$ may 
% be bounded by uniform convergence results from classical empirical process 
% theory \citep{boucheron,bartlett03rademacher}; it is typically 
% of order $O(1/\sqrt{n})$, closely related to the number of samples $n$. The size of $\nu$ also determines the degree of tolerance of poor local minima in $f$; intuitively, from Figure \ref{fig:intro}a, one can see that the smaller $\nu$ is, the `shallower' the spurious local minima in $f$ has to be.

%Fortunately, the empirical risk is often close in function value to another function that has a good landscape for optimization, even though their higher order derivatives may be far apart. For example, the empirical risk is typically pointwise close to the population risk and in some cases, one can show that the population risk is smooth and has no spurious local minima  \citep{brutzkus17globally, li2017convergence}. This implies that any local minima present in the empirical risk must be relatively `shallow', depending on how far it is from a well-behaved target function. Can we escape such local minima? This motivates the central problem in this paper, formally stated as follows.
%
%In the statistical learning setting, 
%
%\cnote{Put this formulation in second paragraph, and say our objective is that if our given function $F$is close to some smooth function $f$, we want to escape those ``sharp'' local minima, and find those local minima persist in the smooth function.}

The key quantity in Problem \eqref{eq:problem_intro} is how much error $\nu$ we can tolerate. An algorithm that can tolerate larger $\nu$ also  escapes `deeper' local minima.  In the context of ERM, this means we require fewer samples to have the same guarantee on avoiding local minima.
To escape shallow local minima in the form of Problem \eqref{eq:problem_intro}, most previous work are based on ideas related to sampling %Most previous work on Problem \eqref{eq:problem_intro} resort to significant noise to escape local minima,  under sampling-based algorithms 
such as simulated annealing \citep{belloni2015escaping} and stochastic gradient Langevin dynamics (SGLD) \citep{zhang2017hitting}. %Such algorithms asymptotically converge to stationary distributions instead of the vicinity around local optima. Moreover, 
%I'm not sure if we should mention this as our algorithm also asymptotically converge to stationary distributions because we fix a step size. We can of course decrease our step size slowly but the sampling algorithms can also lower the temperature slowly.
These techniques require the algorithm to add a significant amount of noise in the optimization procedure, and asymptotically converge to stationary distributions instead of the vicinity around local optima. %Such extra noise could hurt the convergence of the algorithms and does not allow them to escape deeper local minima: 
The only existing work that does not assume $F$ to be convex \citep{zhang2017hitting}, requires error $\nu$ to smaller than $O(\epsilon^2/d^8)$ where $\epsilon$ is the precision of the optimization guarantee (see Definition \ref{def:exactSOSP}) and $d$ is the problem dimension (see Figure~\ref{fig:contri} for a full comparison). 
% Most existing work has tackled this problem in the setting where $F$ is 
% convex \citep{belloni2015escaping,singer15information,risteski16alg}. 
% \citet{zhang2017hitting} showed how to solve the nonconvex version of 
% the problem using a sampling-based algorithm with suboptimal guarantees. Specifically, their algorithm requires $\nu$ to be have the order $\epsilon^2/d^8$ where $\epsilon$ is the precision of the optimization guarantee (see Definition \ref{def:exactSOSP}) and $d$ is the problem dimension (see Figure~\ref{fig:contri}). Hence the algorithm can only escape extremely `shallow' local minima in $f$. In addition, the sampling-based algorithm adds Gaussian noise to the iterates, and converges asymptotically to a stationary distribution. In contrast, an algorithm based on stochastic gradient descent only adds a small amount of perturbation and asymptotically converges to a neighborhood around the local minimum. 
%\cnote{Talk about deep first then Yuchen's work}


We would thus like to answer the two central questions: \textbf{ 1) Can a simple, optimization-based algorithm also avoid shallow local minima?
2) Can we tolerate larger error $\nu$, thus escaping `deeper' local minima? What is the largest error that the best algorithm can tolerate?} 

%Thus we would like to find the dependency of the quality of 
%the solution on  $\nu$. This raises the following central question:
%
%\textbf{How much error $\nu$ can we tolerate to (1) identify the approximate 
%	local minima (see Definition \ref{def:exactSOSP}) of $F$; and (2) efficiently 
%	find the approximate local minima of $F$? } Also, in the latter scenario, can a 
%simple algorithm such as stochastic gradient descent (SGD) achieve this goal?
 % on this approach. 
% study this optimization problem assuming target function $F$ is convex;
%the only work \citep{zhang2017hitting} that can solve this optimization problem in the nonconvex setting relies on a sampling-based method known as Stochastic Gradient Langevin Dynamics (SGLD) \citep{welling11bayesian}. To get an $\epsilon$-approximate solution (see Definition~\ref{def:SOSP}), \citet{zhang2017hitting} can only tolerate a very small function error $\nu = O(\epsilon^2/d^8)$
%\footnote{We note the difference between $\nu$ claimed here and $\nu = O(\epsilon^2)$ claimed in \citep{zhang2017hitting} is due to difference in assumptions. This paper assume Hessian Lipschitz with respect to the standard spectral norm; \citet{zhang2017hitting} assume it with respect to nuclear norm, with their Hessian Lipschitz constant naturally depends on dimension $d$.} with many technical assumptions tailored for sampleing-based algorithms.

%\cnote{Change up to here.}

In this paper, we answer both questions in the affirmative, and establish optimal dependencies between the error $\nu$ and the precision of a solution~$\epsilon$. 
We propose a simple algorithm based on 
SGD (Algorithm~\ref{algo:PSGD}) that is guaranteed to find an approximate 
local minimum of $F$ efficiently if $\nu \le O(\epsilon^{1.5}/d)$, 
thus escaping all saddle points of $F$ and all additional local minima 
introduced by $f$. Moreover, we provide a matching lower bound (up to logarithmic factors) for all algorithms making a polynomial number of queries of $f$.
% showing whenever $\nu \ge \tilde{\Omega}(\epsilon^{1.5}/d)$, no algorithm can successfully achieve above objective within polynomial number of queries to $f$ in the worst case, 
The lower bound shows that our algorithm achieves the optimal tradeoff between $\nu$ and $\epsilon$, as well as the optimal dependence on dimension $d$.
%, among all algorithms making a 
%polynomial number of queries.
% give a simple optimization algorithm based on SGD (Algorithm~\ref{algo:PSGD}) that can achieve the optimal trade-off between $\nu$ and $\epsilon$, as well as the optimal dependence on problem dimension $d$, among all algorithms making polynomial number of queries. 
We also consider the information-theoretic limit for identifying an approximate local 
minimum of $F$ regardless of the number of queries. We give a sharp information-theoretic 
threshold: $\nu = \Theta(\epsilon^{1.5})$ (see Figure~\ref{fig:contri}). 

As a concrete example of the application to minimizing population risk, we show 
that our results can be directly used to give sample complexities for learning 
a ReLU unit, whose empirical risk is nonsmooth while population risk is smooth almost everywhere.  We note that other applications of our framework include two-stage robust 
optimization and private learning (see Section \ref{sec:otherapplications}). 
In these settings, $\nu$ can be viewed as the amount of adversarial perturbation 
or noise due to sources other than data sampling.
%
%
%The standard approach to controlling the effect of the differences between these
%risks requires a combination of statistical guarantees and algorithmic guarantees 
%from optimization: the former focuses on the connection between population risk 
%and empirical risk, and in particular the connection between the empirical risk 
%minimizer (ERM) and the population risk minimizer, while 
%the latter focuses on the empirical risk and tries to guarantee that an ERM
%can be found. Such analyses are much less straightforward in the nonconvex 
%setting notably because empirical risk minimization is not guaranteed when the 
%loss $L$ is nonconvex. Indeed, recent results in nonconvex 
%optimization \citep[e.g.,][]{ge2015escaping, carmon16accelerated,agarwal17finding,jin17escape} generally require that the objective function is smooth and has no spurious 
%local minima. These properties tend to hold only for the population risk, but 
%not for the empirical risk.%In many settings these algorithms cannot be directly applied to obtain ERM as empirical risk can be nonsmooth and have spurious local minima. 
%
%
%The landscape of empirical risk for nonconvex losses can be rough even when 
%the underlying population risk is smooth, as illustrated in Figure \ref{fig:intro}.  Indeed,
%the empirical risk can be nonsmooth in an entire subspace while the population 
%risk is smooth except at a single point (e.g., for convolution networks with 
%Gaussian inputs \citep{brutzkus17globally}), and sampling can introduce 
%exponentially many spurious local minima \citep{auer96exponentially}. 
%In the context of deep learning, many researchers turn to studying the 
%population risk \citep{brutzkus17globally, li2017convergence} while analysis
%of its finite-sample version remains elusive. Even in low-rank matrix problems 
%where analysis of the population risk is straightforward, the analysis of the 
%empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}. 
%
%Our goal in this paper is to show how to design algorithms that, despite 
%only having access to the rough empirical risk, can still optimize the population 
%risk efficiently. Our approach guarantees convergence in population risk with 
%minimal assumptions on its regularity, thus helping to bridge the gap between 
%statistics and nonconvex optimization. 
%As long as the population risk has a well-behaved landscape and is close to the empirical risk in function value, 
%In order to achieve our goal, we design algorithms that are robust to  the differences between population and empirical risk, so that nice population risk can already guarantee the success of optimization algorithm despite the possible bad landscape of empirical loss. 


%
%Nonconvex optimization has become a core topic in modern machine learning. It has wide applications including deep neural networks, reinforcement learning, matrix/tensor factorizations and Bayesian inference. %Traditional nonconvex optimization focus on finding stationary points which can be local minima, local maxima, or even saddle points []. While recent line of works
%Understanding the convergence rates and properties for nonconvex optimization algorithms received a lot of recent attention. In particular, a line of work  \citep{jin17escape, ge2015escaping} showed how to deal with saddle points and converge to local minima efficiently. Getting to a local minimum is also shown to be sufficient for many practical problems \cite{}.
%
%All the nonconvex optimization algorithms mentioned before require access to accurate estimates of function value and its gradient. However, in many statistical applications, the gradient information may not be available, and even the function value can be hard/costly to estimate. In this paper we focus on a {\em robust optimization} problem: 
%Here $\nu$ can be viewed as amount of adversarial perturbation or a measure of uncertainty over the function values of $F$. Given access to $f$, the goal is to find a point that is an approximate local minimum of $F$. %This setting 
%while $F$ is assumed to be smooth, $f$ can be highly-nonsmooth and introduing many additional shallow local minima (see Figure \ref{fig:intro}). Quantitaty $\nu$ can be viewed as adversarial perturbation to true function $F$. The objective of this paper is to find the second-order stationary point (also called approximate local minima) of $F$ satisfying $\grad F(\x) = 0$ and $\hess F(\x) \succeq 0$, thus escaping all the shallow local minima introduced by $f$.


%This general problem has many applications. For example, consider a statistical learning problem with a nonconvex loss function $L_w(x,y)$ for each sample $(x,y)\sim \D$. What we really want to optimize is the population loss $F(w) = \E_{(x,y)\sim \D}[L_w(x,y)]$. However, what we have access to is the empirical loss, which is just the average over the training examples. For many choices of $L$ (e.g. a 0/1 classification loss) even though $F$ can be well-behaved, $f$ is highly non-smooth and we can only guarantee the point-wise closeness of the two functions (see Figure~\ref{fig:intro}). In this setting the uncertainty $\nu$ is closely related to the number of samples, and we would like to get tight dependencies between $\nu$ and the quality of solution. % where $F$ is the population loss, typically nice-behaved due to its averaging nature; $f$ is the empirical loss, typically highly non-smooth and can introduce many additional shallow local minima. The point-wise closeness of $(F, f)$ is guaranteed by standard uniform convergence results []. 


%
%
%The central questions in this problem are \textbf{how much perturbation $\nu$ can we tolerate to 1) identify the SOSP of $F$; 2) efficiently find the SOSP of $F$? and in latter scenario, can simple algorithm such as SGD achieve this goal?}
%
%There has been many researches under this general framework in recent years (e.g. \citep{belloni2015escaping,singer15information,risteski16alg}), however, this line of works has been focused on the special case where underlying function $F$ is convex, and the objective is to find the global optimal of $F$. For general nonconvex $F$, \citet{zhang2017hitting} proposed a sampling based algorithm---stochastic gradient Langevin dynamics (SGLD), and proved that algorithm will succeed if perturbation is small $\nu \le O(\epsilon^{2}/d^8)$. It remains unclear if this small perturbation level is necessary to guarantee escaping shallow local minima.
%
%In this work, we proposed a simple optimization based algorithm --- zero-th order stochastic gradient descent, showing if finds the SOSP of $F$ and thus escaping all shallow local minima of $f$ given perturbation $\nu \le O(\epsilon^{1.5}/d)$, allowing significant more perturbation compared to previous work. On the other hand, we also proved while it is information-theoretical impossible to identify the SOSP of $F$ if $\nu \ge \Omega(\epsilon^{1.5})$, no polynomial algorithm can find the SOSP of $F$ if
%$\nu \ge \tilde{\Omega}(\epsilon^{1.5}/d)$ matching the noise tolerance of our SGD algorithm up to logarithmic factors.

%\cnote{Maybe use real line axis, think about exponential learnable or not learnable}
%\cnote{Say something about the techniques and examples}
%\cnote{Say difference between Langevin and our algorithm}
%
%\lnote{Notes from meeting with Mike (Feb 13). There has been a lot of progress in convex and nonconvex optimization, but not enough attention has been paid to the interplay between statistics and optimization. In particular, gradient based methods often assume that the objective function being optimized is well-behaved (smooth, no local minima) when oracles only have access to a less well-behaved \emph{approximation} to the true objective. This may be due to sampling, privacy or  nested objectives (e.g. in robust optimization formulations). Stochasticity in optimization introduces a problem where the exact objective is not known. The approximate objective function may have a rough surface with a drastically different differential landscape, so the guarantees of many sophisticated gradient and Hessian-based optimization methods no longer hold in this setting. Moreover, sampling can introduce shallow local minima. Our work takes a step towards bridging this gap between optimization theory and statistics.}


\begin{figure}[t]
\centering
\includegraphics[width=.9\textwidth]{contribution3.png}
\caption{Complete characterization of error $\nu$ vs accuracy $\epsilon$ and dimension $d$.} \label{fig:contri}
\end{figure}

% What is the completeness characterization of $\nu$ vs the hardness?
% Is gradient Langevin (or sampling based algorithm) necessary to solve this problem?








% \textbf{Conjecture:}
% \begin{itemize}
% 	\item Given zero-th order oracle $f(\x)$ so that $\sup_{\x}|f(\x) - F(\x)| \le \poly(\epsilon, \frac{1}{d})$, 
% 	where $F$ is $\ell$-gradient Lipschitz and $\rho$-Hessian Lipschitz. Then, stochastic gradient with perturbation will find second-order stationary point of $F$ in $\poly(\epsilon, d)$ iterations.
% \end{itemize}


% % \item Given first order oracle $\g(\x)$ so that $\sup_{\x} \norm{\g(\x) - \grad F(\x)} \le \poly(\epsilon, \frac{1}{d})$,
% % perturbed gradient descent (with $\g(\x)$) will find second order stationary point of $F$ with sharper rate.


% \textbf{Goal:}
% \begin{itemize}
% 	\item Finding second-order stationary with zero-th order oracle (rate).
% 	\item Finding second-order stationary with zero-th order oracle of point-wise close function (rate).
% 	Describe what are the additional local minima, and how smoothing technique removes them. 
% 	\item Connection to \citep{belloni2015escaping,zhang2017hitting,mei2016landscape,loh2013regularized}
% 	\begin{itemize}
% 		\item \citet{belloni2015escaping}: Assume F is (strongly) convex. Compare their result to our smoothing + SGD strategy, in terms of the $d$ and $\epsilon$ dependence in the iteration complexity and $\nu$.
% 		\item \citet{mei2016landscape}: Assume $f$ (or equivalently the loss function in statistical learning) is differentiable. They have results for gradient and Hessian difference without smoothing.
% 	\end{itemize}
% \end{itemize}

% \textbf{Contribution:}
% \begin{itemize}
% 	\item Removing a lot of redundant assumptions. State better results in a cleaner way.
% 	\item Show given this closeness to a good function (application in statistical setting), sampling based algorithm is not necessary for escaping shallow local minima. Optimization based approaches can achieve same/better guarantee much faster speed.
% 	\item First zero-th order result?
% \end{itemize}

% \textbf{Main application:}
% \begin{itemize}
% 	\item Empirical loss vs population loss, uniform convergence
% \end{itemize}

\input{related}


==> introduction-backup.tex <==
% !TeX root = main.tex 

\section{Introduction}

The use of nonconvex loss functions has been essential in modern machine learning. A further ingredient has been the use of efficient gradient-based optimization. This has strongly motivated gradient-based optimization algorithms that have provable guarantees for nonconvex functions. Unlike convex functions that usually have a unique critical point that is both locally and globally minimal, a nonconvex function can have many local maxima, local minima and saddle points. Finding global minima is NP-hard in general. In some applications \cite[e.g.][]{bhoj16global, ge2016matrix}, all the local minima are desirable solutions, while saddle points are not acceptable. Indeed, recent results in nonconvex optimization \citep[e.g.,][]{ge2015escaping, carmon16accelerated,agarwal17finding,jin17escape} guarantee avoiding saddle points when the objective function is smooth. However, in practical learning problems, one often encounters functions that are nonsmooth and have undesirable local minima, in which case these guarantees are no longer applicable.
%Two key obstables to this are saddle points and local minima with suboptimal loss. 

Since one cannot hope to deal with arbitrarily bad local minima and nonsmoothness, this paper is concerned with resolving an important class of spurious local minima that arises naturally in nonconvex \textit{empirical risk minimization}. Given a nonconvex loss function $L(\btheta; \z)$ and data $\z_i$ sampled from 
an underlying distribution $\D$, the population risk $\poploss$ and empirical 
risk $\emploss$ are defined as follows:
\begin{equation*}
	\poploss(\btheta) = \E_{\z \sim \D}[L(\btheta; \z)], \qquad \emploss(\btheta) = \frac{1}{n}\sum_{i=1}^n L(\btheta; \z_i).
\end{equation*}

\lnote{can we make the above inline?}
While one would like to find the model parameter $\btheta$ that minimizes population risk, learning algorithms only have access to empirical risk, which is the average loss over training examples. In many cases, the empirical risk is known to have a landscape that is problematic for optimization. For example, in the context of deep learning, the empirical risk can be nonsmooth in an entire subspace for convolution networks with 
Gaussian inputs \citep{brutzkus17globally}, or have many spurious local minima due to finite sampling \citep{auer96exponentially} (as illustrated in Figure \ref{fig:intro} b). In other cases, the empirical risk can be intractable to analyze, making it difficult to rule out the existence of poor local minima. Even in low-rank matrix problems 
where analysis of the population risk is straightforward, the analysis of the 
empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}.  


\begin{figure}[t]
	\centering
	\includegraphics[width=0.3\textwidth, trim=80 70 240 10, clip]{nu_example.pdf}%
	\includegraphics[width=0.35\textwidth, trim=0 30 0 10, clip]{intro_pop}%
	\includegraphics[width=0.35\textwidth, trim=0 30 0 10, clip]{intro_emp}
	\caption{a) Function error $\nu$; b) Population risk vs empirical risk} \label{fig:intro}
\end{figure}

Fortunately, the empirical risk is often close in function value to another function that has a good landscape for optimization, even though their higher order derivatives may be far apart. For example, the empirical risk is typically pointwise close to the population risk and in some cases, one can show that the population risk is smooth and has no spurious local minima  \citep{brutzkus17globally, li2017convergence}. This implies that any local minima present in the empirical risk must be relatively `shallow', depending on how far it is from a well-behaved target function. Can we escape such local minima? This motivates the central problem in this paper, formally stated as follows.

Suppose that we want to optimize a target function $F$, but only 
have access to an observed function $f$ that is close to $F$ pointwise:
\begin{equation*}
\norm{F - f}_{\infty} \le \nu. 
\end{equation*}
In the statistical learning setting, $(F, f)$ might be the population and 
empirical risk, $(\poploss, \emploss)$.  The function error $\nu$ can be 
viewed as a measure of uncertainty over the function value of $F$, which may 
be bounded by uniform convergence results from classical empirical process 
theory \citep{boucheron,bartlett03rademacher}. The error $\nu$ is typically 
of order $O(1/\sqrt{n})$, closely related to the number of samples $n$. 


Most existing work has tackled this problem in the setting where $F$ is 
convex \citep{belloni2015escaping,singer15information,risteski16alg}. 
\citet{zhang2017hitting} show how to solve the nonconvex version of 
the problem using a sampling-based algorithm with suboptimal guarantees. Specifically, their algorithm requires $\nu$ to be have the order $\epsilon^2/d^8$ where $\epsilon$ is the precision of the optimization guarantee (see Definition \ref{def:exactSOSP}) and $d$ is the problem dimension (see Figure~\ref{fig:contri}). This puts a stringent restriction on the types of poor local minima in $f$ that the algorithm can tolerate; intuitively from Figure \ref{fig:intro}a, one can see that the larger $\nu$ is, the deeper the spurious local minima in $f$ is allowed to be. In addition, the sampling-based algorithm adds Gaussian noise to the iterates, and converges asymptotically to a stationary distribution. In contrast, an algorithm based on stochastic gradient descent only adds a small amount of perturbation and asymptotically converges to a neighborhood around the local minimum. 

Therefore we would like to answer the two central questions: \textbf{ 1) Given a larger $\nu$, can we still guarantee finding approximate local minima of $F$ thus escaping all spurious local minima in $f$? and 2) Can a simple, non-sampling-based algorithm achieve such a guarantee? } 

%Thus we would like to find the dependency of the quality of 
%the solution on  $\nu$. This raises the following central question:
%
%\textbf{How much error $\nu$ can we tolerate to (1) identify the approximate 
%	local minima (see Definition \ref{def:exactSOSP}) of $F$; and (2) efficiently 
%	find the approximate local minima of $F$? } Also, in the latter scenario, can a 
%simple algorithm such as stochastic gradient descent (SGD) achieve this goal?
 % on this approach. 
% study this optimization problem assuming target function $F$ is convex;
%the only work \citep{zhang2017hitting} that can solve this optimization problem in the nonconvex setting relies on a sampling-based method known as Stochastic Gradient Langevin Dynamics (SGLD) \citep{welling11bayesian}. To get an $\epsilon$-approximate solution (see Definition~\ref{def:SOSP}), \citet{zhang2017hitting} can only tolerate a very small function error $\nu = O(\epsilon^2/d^8)$
%\footnote{We note the difference between $\nu$ claimed here and $\nu = O(\epsilon^2)$ claimed in \citep{zhang2017hitting} is due to difference in assumptions. This paper assume Hessian Lipschitz with respect to the standard spectral norm; \citet{zhang2017hitting} assume it with respect to nuclear norm, with their Hessian Lipschitz constant naturally depends on dimension $d$.} with many technical assumptions tailored for sampleing-based algorithms.

In this paper, we establish optimal dependencies between the error $\nu$ and 
the precision of a solution~$\epsilon$. We propose a simple algorithm based on 
SGD (Algorithm~\ref{algo:PSGD}) which is guaranteed to find approximate 
local minima of $F$ efficiently if $\nu \le O(\epsilon^{1.5}/d)$, 
thus escaping all saddle points of $F$ and all the additional local minima 
introduced by $f$. Moreover, we provide a matching lower bound (up to logarithmic factors) for all algorithms making a polynomial number of queries.
% showing whenever $\nu \ge \tilde{\Omega}(\epsilon^{1.5}/d)$, no algorithm can successfully achieve above objective within polynomial number of queries to $f$ in the worst case, 
The lower bound shows that our algorithm achieves the optimal trade-off between $\nu$ and $\epsilon$, as well as the optimal dependence on problem dimension $d$.
%, among all algorithms making a 
%polynomial number of queries.
% give a simple optimization algorithm based on SGD (Algorithm~\ref{algo:PSGD}) that can achieve the optimal trade-off between $\nu$ and $\epsilon$, as well as the optimal dependence on problem dimension $d$, among all algorithms making polynomial number of queries. 
We also consider an information-theoretic limit to identify a approximate local 
minimum of $F$ regardless of the number of queries. We give a sharp information-theoretic 
threshold $\nu = \Theta(\epsilon^{1.5})$ (see Figure~\ref{fig:contri}). 

As a concrete example of the application to minimizing population risk, we will show 
that our results can be directly used to give sample complexities for learning 
a ReLU unit, whose empirical risk is nonsmooth.  We note that other applications 
of our framework include learning with missing or corrupted data, two-stage robust 
optimization and private learning (see Section \ref{sec:otherapplications}). 
In these settings, $\nu$ can be viewed as the amount of adversarial perturbation 
or noise due to sources other than data sampling.
%
%
%The standard approach to controlling the effect of the differences between these
%risks requires a combination of statistical guarantees and algorithmic guarantees 
%from optimization: the former focuses on the connection between population risk 
%and empirical risk, and in particular the connection between the empirical risk 
%minimizer (ERM) and the population risk minimizer, while 
%the latter focuses on the empirical risk and tries to guarantee that an ERM
%can be found. Such analyses are much less straightforward in the nonconvex 
%setting notably because empirical risk minimization is not guaranteed when the 
%loss $L$ is nonconvex. Indeed, recent results in nonconvex 
%optimization \citep[e.g.,][]{ge2015escaping, carmon16accelerated,agarwal17finding,jin17escape} generally require that the objective function is smooth and has no spurious 
%local minima. These properties tend to hold only for the population risk, but 
%not for the empirical risk.%In many settings these algorithms cannot be directly applied to obtain ERM as empirical risk can be nonsmooth and have spurious local minima. 
%
%
%The landscape of empirical risk for nonconvex losses can be rough even when 
%the underlying population risk is smooth, as illustrated in Figure \ref{fig:intro}.  Indeed,
%the empirical risk can be nonsmooth in an entire subspace while the population 
%risk is smooth except at a single point (e.g., for convolution networks with 
%Gaussian inputs \citep{brutzkus17globally}), and sampling can introduce 
%exponentially many spurious local minima \citep{auer96exponentially}. 
%In the context of deep learning, many researchers turn to studying the 
%population risk \citep{brutzkus17globally, li2017convergence} while analysis
%of its finite-sample version remains elusive. Even in low-rank matrix problems 
%where analysis of the population risk is straightforward, the analysis of the 
%empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}. 
%
%Our goal in this paper is to show how to design algorithms that, despite 
%only having access to the rough empirical risk, can still optimize the population 
%risk efficiently. Our approach guarantees convergence in population risk with 
%minimal assumptions on its regularity, thus helping to bridge the gap between 
%statistics and nonconvex optimization. 
%As long as the population risk has a well-behaved landscape and is close to the empirical risk in function value, 
%In order to achieve our goal, we design algorithms that are robust to  the differences between population and empirical risk, so that nice population risk can already guarantee the success of optimization algorithm despite the possible bad landscape of empirical loss. 


%
%Nonconvex optimization has become a core topic in modern machine learning. It has wide applications including deep neural networks, reinforcement learning, matrix/tensor factorizations and Bayesian inference. %Traditional nonconvex optimization focus on finding stationary points which can be local minima, local maxima, or even saddle points []. While recent line of works
%Understanding the convergence rates and properties for nonconvex optimization algorithms received a lot of recent attention. In particular, a line of work  \citep{jin17escape, ge2015escaping} showed how to deal with saddle points and converge to local minima efficiently. Getting to a local minimum is also shown to be sufficient for many practical problems \cite{}.
%
%All the nonconvex optimization algorithms mentioned before require access to accurate estimates of function value and its gradient. However, in many statistical applications, the gradient information may not be available, and even the function value can be hard/costly to estimate. In this paper we focus on a {\em robust optimization} problem: 
%Here $\nu$ can be viewed as amount of adversarial perturbation or a measure of uncertainty over the function values of $F$. Given access to $f$, the goal is to find a point that is an approximate local minimum of $F$. %This setting 
%while $F$ is assumed to be smooth, $f$ can be highly-nonsmooth and introduing many additional shallow local minima (see Figure \ref{fig:intro}). Quantitaty $\nu$ can be viewed as adversarial perturbation to true function $F$. The objective of this paper is to find the second-order stationary point (also called approximate local minima) of $F$ satisfying $\grad F(\x) = 0$ and $\hess F(\x) \succeq 0$, thus escaping all the shallow local minima introduced by $f$.


%This general problem has many applications. For example, consider a statistical learning problem with a nonconvex loss function $L_w(x,y)$ for each sample $(x,y)\sim \D$. What we really want to optimize is the population loss $F(w) = \E_{(x,y)\sim \D}[L_w(x,y)]$. However, what we have access to is the empirical loss, which is just the average over the training examples. For many choices of $L$ (e.g. a 0/1 classification loss) even though $F$ can be well-behaved, $f$ is highly non-smooth and we can only guarantee the point-wise closeness of the two functions (see Figure~\ref{fig:intro}). In this setting the uncertainty $\nu$ is closely related to the number of samples, and we would like to get tight dependencies between $\nu$ and the quality of solution. % where $F$ is the population loss, typically nice-behaved due to its averaging nature; $f$ is the empirical loss, typically highly non-smooth and can introduce many additional shallow local minima. The point-wise closeness of $(F, f)$ is guaranteed by standard uniform convergence results []. 


%
%
%The central questions in this problem are \textbf{how much perturbation $\nu$ can we tolerate to 1) identify the SOSP of $F$; 2) efficiently find the SOSP of $F$? and in latter scenario, can simple algorithm such as SGD achieve this goal?}
%
%There has been many researches under this general framework in recent years (e.g. \citep{belloni2015escaping,singer15information,risteski16alg}), however, this line of works has been focused on the special case where underlying function $F$ is convex, and the objective is to find the global optimal of $F$. For general nonconvex $F$, \citet{zhang2017hitting} proposed a sampling based algorithm---stochastic gradient Langevin dynamics (SGLD), and proved that algorithm will succeed if perturbation is small $\nu \le O(\epsilon^{2}/d^8)$. It remains unclear if this small perturbation level is necessary to guarantee escaping shallow local minima.
%
%In this work, we proposed a simple optimization based algorithm --- zero-th order stochastic gradient descent, showing if finds the SOSP of $F$ and thus escaping all shallow local minima of $f$ given perturbation $\nu \le O(\epsilon^{1.5}/d)$, allowing significant more perturbation compared to previous work. On the other hand, we also proved while it is information-theoretical impossible to identify the SOSP of $F$ if $\nu \ge \Omega(\epsilon^{1.5})$, no polynomial algorithm can find the SOSP of $F$ if
%$\nu \ge \tilde{\Omega}(\epsilon^{1.5}/d)$ matching the noise tolerance of our SGD algorithm up to logarithmic factors.

%\cnote{Maybe use real line axis, think about exponential learnable or not learnable}
%\cnote{Say something about the techniques and examples}
%\cnote{Say difference between Langevin and our algorithm}
%
%\lnote{Notes from meeting with Mike (Feb 13). There has been a lot of progress in convex and nonconvex optimization, but not enough attention has been paid to the interplay between statistics and optimization. In particular, gradient based methods often assume that the objective function being optimized is well-behaved (smooth, no local minima) when oracles only have access to a less well-behaved \emph{approximation} to the true objective. This may be due to sampling, privacy or  nested objectives (e.g. in robust optimization formulations). Stochasticity in optimization introduces a problem where the exact objective is not known. The approximate objective function may have a rough surface with a drastically different differential landscape, so the guarantees of many sophisticated gradient and Hessian-based optimization methods no longer hold in this setting. Moreover, sampling can introduce shallow local minima. Our work takes a step towards bridging this gap between optimization theory and statistics.}


\begin{figure}[t]
\centering
\includegraphics[width=.9\textwidth]{contribution3.png}
\caption{Complete characterization of error $\nu$ vs accuracy $\epsilon$ and dimension $d$.} \label{fig:contri}
\end{figure}

% What is the completeness characterization of $\nu$ vs the hardness?
% Is gradient Langevin (or sampling based algorithm) necessary to solve this problem?








% \textbf{Conjecture:}
% \begin{itemize}
% 	\item Given zero-th order oracle $f(\x)$ so that $\sup_{\x}|f(\x) - F(\x)| \le \poly(\epsilon, \frac{1}{d})$, 
% 	where $F$ is $\ell$-gradient Lipschitz and $\rho$-Hessian Lipschitz. Then, stochastic gradient with perturbation will find second-order stationary point of $F$ in $\poly(\epsilon, d)$ iterations.
% \end{itemize}


% % \item Given first order oracle $\g(\x)$ so that $\sup_{\x} \norm{\g(\x) - \grad F(\x)} \le \poly(\epsilon, \frac{1}{d})$,
% % perturbed gradient descent (with $\g(\x)$) will find second order stationary point of $F$ with sharper rate.


% \textbf{Goal:}
% \begin{itemize}
% 	\item Finding second-order stationary with zero-th order oracle (rate).
% 	\item Finding second-order stationary with zero-th order oracle of point-wise close function (rate).
% 	Describe what are the additional local minima, and how smoothing technique removes them. 
% 	\item Connection to \citep{belloni2015escaping,zhang2017hitting,mei2016landscape,loh2013regularized}
% 	\begin{itemize}
% 		\item \citet{belloni2015escaping}: Assume F is (strongly) convex. Compare their result to our smoothing + SGD strategy, in terms of the $d$ and $\epsilon$ dependence in the iteration complexity and $\nu$.
% 		\item \citet{mei2016landscape}: Assume $f$ (or equivalently the loss function in statistical learning) is differentiable. They have results for gradient and Hessian difference without smoothing.
% 	\end{itemize}
% \end{itemize}

% \textbf{Contribution:}
% \begin{itemize}
% 	\item Removing a lot of redundant assumptions. State better results in a cleaner way.
% 	\item Show given this closeness to a good function (application in statistical setting), sampling based algorithm is not necessary for escaping shallow local minima. Optimization based approaches can achieve same/better guarantee much faster speed.
% 	\item First zero-th order result?
% \end{itemize}

% \textbf{Main application:}
% \begin{itemize}
% 	\item Empirical loss vs population loss, uniform convergence
% \end{itemize}

\input{related}


==> introduction-old.tex <==
% !TeX root = main.tex 

\section{Introduction}

The use of nonconvex loss functions has been essential in modern machine learning. 
A further essential ingredient has been the use of gradient-based optimization.


But there is a disconnect---in the theory of gradient-based optimization, for
both nonconvex and convex functions, concepts such as smoothness and strong 
convexity play an important role in the theory.  However, while the population 
risk may have such simplifying properties, these properties will generally be 
destroyed by the sampling process that leads to the empirical risk.  This
disconnect between population risk and empirical risk is particularly glaring 
in the nonconvex setting.

Given a nonconvex loss function $L(\btheta; \z)$ and data $\z_i$ sampled from 
an underlying distribution $\D$, the population risk $\poploss$ and empirical 
risk $\emploss$ are defined as follows:
\begin{equation*}
\poploss(\btheta) = \E_{\z \sim \D}[L(\btheta; \z)], \qquad \emploss(\btheta) = \frac{1}{n}\sum_{i=1}^n L(\btheta; \z_i).
\end{equation*}
The standard approach to controlling the effect of the differences between these
risks requires a combination of statistical guarantees and algorithmic guarantees 
from optimization: the former focuses on the connection between population risk 
and empirical risk, and in particular the connection between the empirical risk 
minimizer (ERM) and the population risk minimizer, while 
the latter focuses on the empirical risk and tries to guarantee that an ERM
can be found. Such analyses are much less straightforward in the nonconvex 
setting notably because empirical risk minimization is not guaranteed when the 
loss $L$ is nonconvex. Indeed, recent results in nonconvex 
optimization \citep[e.g.,][]{ge2015escaping, carmon16accelerated,agarwal17finding,jin17escape} generally require that the objective function is smooth and has no spurious 
local minima. These properties tend to hold only for the population risk, but 
not for the empirical risk.%In many settings these algorithms cannot be directly applied to obtain ERM as empirical risk can be nonsmooth and have spurious local minima. 

\begin{figure}[t]
    \centering
    \includegraphics[width=0.41\textwidth, trim=0 30 0 10, clip]{intro_pop}
    \includegraphics[width=0.41\textwidth, trim=0 30 0 10, clip]{intro_emp}
    \caption{Population risk vs empirical risk} \label{fig:intro}
\end{figure}

The landscape of empirical risk for nonconvex losses can be rough even when 
the underlying population risk is smooth, as illustrated in Figure \ref{fig:intro}.  Indeed,
the empirical risk can be nonsmooth in an entire subspace while the population 
risk is smooth except at a single point (e.g., for convolution networks with 
Gaussian inputs \citep{brutzkus17globally}), and sampling can introduce 
exponentially many spurious local minima \citep{auer96exponentially}. 
In the context of deep learning, many researchers turn to studying the 
population risk \citep{brutzkus17globally, li2017convergence} while analysis
of its finite-sample version remains elusive. Even in low-rank matrix problems 
where analysis of the population risk is straightforward, the analysis of the 
empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}. 

Our goal in this paper is to show how to design algorithms that, despite 
only having access to the rough empirical risk, can still optimize the population 
risk efficiently. Our approach guarantees convergence in population risk with 
minimal assumptions on its regularity, thus helping to bridge the gap between 
statistics and nonconvex optimization. 
%As long as the population risk has a well-behaved landscape and is close to the empirical risk in function value, 
%In order to achieve our goal, we design algorithms that are robust to  the differences between population and empirical risk, so that nice population risk can already guarantee the success of optimization algorithm despite the possible bad landscape of empirical loss. 

Concretely, suppose that we want to optimize a target function $F$, but only 
have access to an observed function $f$ that is close to $F$ pointwise:
\begin{equation*}
\norm{F - f}_{\infty} \le \nu. 
\end{equation*}
In the statistical learning setting, $(F, f)$ might be the population and 
empirical risk, $(\poploss, \emploss)$.  The function error $\nu$ can be 
viewed as a measure of uncertainty over the function value of $F$, which may 
be bounded by uniform convergence results from classical empirical process 
theory \citep{boucheron,bartlett03rademacher}. The error $\nu$ is typically 
of order $O(1/\sqrt{n})$, closely related to the number of samples $n$. 
Thus we would like to find the dependency of the quality of 
the solution on  $\nu$. This raises the following central question:

\textbf{How much error $\nu$ can we tolerate to (1) identify the approximate 
local minima (see Definition \ref{def:exactSOSP}) of $F$; and (2) efficiently 
find the approximate local minima of $F$? } Also, in the latter scenario, can a 
simple algorithm such as stochastic gradient descent (SGD) achieve this goal?

Most existing work has tackled this problem in the setting where $F$ is 
convex \citep{belloni2015escaping,singer15information,risteski16alg}. 
\citet{zhang2017hitting} show how to solve the nonconvex version of 
the problem using a sampling-based algorithm with suboptimal guarantees (see Section~\ref{sec:related} for further discussion). % on this approach. 
% study this optimization problem assuming target function $F$ is convex;
%the only work \citep{zhang2017hitting} that can solve this optimization problem in the nonconvex setting relies on a sampling-based method known as Stochastic Gradient Langevin Dynamics (SGLD) \citep{welling11bayesian}. To get an $\epsilon$-approximate solution (see Definition~\ref{def:SOSP}), \citet{zhang2017hitting} can only tolerate a very small function error $\nu = O(\epsilon^2/d^8)$
%\footnote{We note the difference between $\nu$ claimed here and $\nu = O(\epsilon^2)$ claimed in \citep{zhang2017hitting} is due to difference in assumptions. This paper assume Hessian Lipschitz with respect to the standard spectral norm; \citet{zhang2017hitting} assume it with respect to nuclear norm, with their Hessian Lipschitz constant naturally depends on dimension $d$.} with many technical assumptions tailored for sampleing-based algorithms.

In this paper, we establish optimal dependencies between the error $\nu$ and 
the accuracy of a solution~$\epsilon$. We propose a simple algorithm based on 
SGD (Algorithm~\ref{algo:PSGD}) which is guaranteed to find approximate 
local minima of $F$ efficiently if $\nu \le O(\epsilon^{1.5}/d)$, 
thus escaping all saddle points of $F$ and all the additional local minima 
introduced by $f$. Moreover, we provide a matching lower bound (up to logarithmic factors) for all algorithms making a polynomial number of queries.
% showing whenever $\nu \ge \tilde{\Omega}(\epsilon^{1.5}/d)$, no algorithm can successfully achieve above objective within polynomial number of queries to $f$ in the worst case, 
The lower bound shows that our algorithm achieves the optimal trade-off between $\nu$ and $\epsilon$, as well as the optimal dependence on problem dimension $d$.
%, among all algorithms making a 
%polynomial number of queries.
% give a simple optimization algorithm based on SGD (Algorithm~\ref{algo:PSGD}) that can achieve the optimal trade-off between $\nu$ and $\epsilon$, as well as the optimal dependence on problem dimension $d$, among all algorithms making polynomial number of queries. 
We also consider an information-theoretic limit to identify a approximate local 
minimum of $F$ regardless of the number of queries. We give a sharp information-theoretic 
threshold $\nu = \Theta(\epsilon^{1.5})$ (see Figure~\ref{fig:contri}). 

As a concrete example of the application to minimizing population risk, we will show 
that our results can be directly used to give sample complexities for learning 
a ReLU unit, whose empirical risk is nonsmooth.  We note that other applications 
of our framework include learning with missing or corrupted data, two-stage robust 
optimization and private learning (see Section \ref{sec:otherapplications}). 
In these settings, $\nu$ can be viewed as the amount of adversarial perturbation 
or noise due to sources other than data sampling.

%
%Nonconvex optimization has become a core topic in modern machine learning. It has wide applications including deep neural networks, reinforcement learning, matrix/tensor factorizations and Bayesian inference. %Traditional nonconvex optimization focus on finding stationary points which can be local minima, local maxima, or even saddle points []. While recent line of works
%Understanding the convergence rates and properties for nonconvex optimization algorithms received a lot of recent attention. In particular, a line of work  \citep{jin17escape, ge2015escaping} showed how to deal with saddle points and converge to local minima efficiently. Getting to a local minimum is also shown to be sufficient for many practical problems \cite{}.
%
%All the nonconvex optimization algorithms mentioned before require access to accurate estimates of function value and its gradient. However, in many statistical applications, the gradient information may not be available, and even the function value can be hard/costly to estimate. In this paper we focus on a {\em robust optimization} problem: 
%Here $\nu$ can be viewed as amount of adversarial perturbation or a measure of uncertainty over the function values of $F$. Given access to $f$, the goal is to find a point that is an approximate local minimum of $F$. %This setting 
%while $F$ is assumed to be smooth, $f$ can be highly-nonsmooth and introduing many additional shallow local minima (see Figure \ref{fig:intro}). Quantitaty $\nu$ can be viewed as adversarial perturbation to true function $F$. The objective of this paper is to find the second-order stationary point (also called approximate local minima) of $F$ satisfying $\grad F(\x) = 0$ and $\hess F(\x) \succeq 0$, thus escaping all the shallow local minima introduced by $f$.


%This general problem has many applications. For example, consider a statistical learning problem with a nonconvex loss function $L_w(x,y)$ for each sample $(x,y)\sim \D$. What we really want to optimize is the population loss $F(w) = \E_{(x,y)\sim \D}[L_w(x,y)]$. However, what we have access to is the empirical loss, which is just the average over the training examples. For many choices of $L$ (e.g. a 0/1 classification loss) even though $F$ can be well-behaved, $f$ is highly non-smooth and we can only guarantee the point-wise closeness of the two functions (see Figure~\ref{fig:intro}). In this setting the uncertainty $\nu$ is closely related to the number of samples, and we would like to get tight dependencies between $\nu$ and the quality of solution. % where $F$ is the population loss, typically nice-behaved due to its averaging nature; $f$ is the empirical loss, typically highly non-smooth and can introduce many additional shallow local minima. The point-wise closeness of $(F, f)$ is guaranteed by standard uniform convergence results []. 


%
%
%The central questions in this problem are \textbf{how much perturbation $\nu$ can we tolerate to 1) identify the SOSP of $F$; 2) efficiently find the SOSP of $F$? and in latter scenario, can simple algorithm such as SGD achieve this goal?}
%
%There has been many researches under this general framework in recent years (e.g. \citep{belloni2015escaping,singer15information,risteski16alg}), however, this line of works has been focused on the special case where underlying function $F$ is convex, and the objective is to find the global optimal of $F$. For general nonconvex $F$, \citet{zhang2017hitting} proposed a sampling based algorithm---stochastic gradient Langevin dynamics (SGLD), and proved that algorithm will succeed if perturbation is small $\nu \le O(\epsilon^{2}/d^8)$. It remains unclear if this small perturbation level is necessary to guarantee escaping shallow local minima.
%
%In this work, we proposed a simple optimization based algorithm --- zero-th order stochastic gradient descent, showing if finds the SOSP of $F$ and thus escaping all shallow local minima of $f$ given perturbation $\nu \le O(\epsilon^{1.5}/d)$, allowing significant more perturbation compared to previous work. On the other hand, we also proved while it is information-theoretical impossible to identify the SOSP of $F$ if $\nu \ge \Omega(\epsilon^{1.5})$, no polynomial algorithm can find the SOSP of $F$ if
%$\nu \ge \tilde{\Omega}(\epsilon^{1.5}/d)$ matching the noise tolerance of our SGD algorithm up to logarithmic factors.

%\cnote{Maybe use real line axis, think about exponential learnable or not learnable}
%\cnote{Say something about the techniques and examples}
%\cnote{Say difference between Langevin and our algorithm}
%
%\lnote{Notes from meeting with Mike (Feb 13). There has been a lot of progress in convex and nonconvex optimization, but not enough attention has been paid to the interplay between statistics and optimization. In particular, gradient based methods often assume that the objective function being optimized is well-behaved (smooth, no local minima) when oracles only have access to a less well-behaved \emph{approximation} to the true objective. This may be due to sampling, privacy or  nested objectives (e.g. in robust optimization formulations). Stochasticity in optimization introduces a problem where the exact objective is not known. The approximate objective function may have a rough surface with a drastically different differential landscape, so the guarantees of many sophisticated gradient and Hessian-based optimization methods no longer hold in this setting. Moreover, sampling can introduce shallow local minima. Our work takes a step towards bridging this gap between optimization theory and statistics.}


\begin{figure}[t]
\centering
\includegraphics[width=.9\textwidth]{contribution3.png}
\caption{Complete characterization of error $\nu$ vs accuracy $\epsilon$ and dimension $d$.} \label{fig:contri}
\end{figure}

% What is the completeness characterization of $\nu$ vs the hardness?
% Is gradient Langevin (or sampling based algorithm) necessary to solve this problem?








% \textbf{Conjecture:}
% \begin{itemize}
% 	\item Given zero-th order oracle $f(\x)$ so that $\sup_{\x}|f(\x) - F(\x)| \le \poly(\epsilon, \frac{1}{d})$, 
% 	where $F$ is $\ell$-gradient Lipschitz and $\rho$-Hessian Lipschitz. Then, stochastic gradient with perturbation will find second-order stationary point of $F$ in $\poly(\epsilon, d)$ iterations.
% \end{itemize}


% % \item Given first order oracle $\g(\x)$ so that $\sup_{\x} \norm{\g(\x) - \grad F(\x)} \le \poly(\epsilon, \frac{1}{d})$,
% % perturbed gradient descent (with $\g(\x)$) will find second order stationary point of $F$ with sharper rate.


% \textbf{Goal:}
% \begin{itemize}
% 	\item Finding second-order stationary with zero-th order oracle (rate).
% 	\item Finding second-order stationary with zero-th order oracle of point-wise close function (rate).
% 	Describe what are the additional local minima, and how smoothing technique removes them. 
% 	\item Connection to \citep{belloni2015escaping,zhang2017hitting,mei2016landscape,loh2013regularized}
% 	\begin{itemize}
% 		\item \citet{belloni2015escaping}: Assume F is (strongly) convex. Compare their result to our smoothing + SGD strategy, in terms of the $d$ and $\epsilon$ dependence in the iteration complexity and $\nu$.
% 		\item \citet{mei2016landscape}: Assume $f$ (or equivalently the loss function in statistical learning) is differentiable. They have results for gradient and Hessian difference without smoothing.
% 	\end{itemize}
% \end{itemize}

% \textbf{Contribution:}
% \begin{itemize}
% 	\item Removing a lot of redundant assumptions. State better results in a cleaner way.
% 	\item Show given this closeness to a good function (application in statistical setting), sampling based algorithm is not necessary for escaping shallow local minima. Optimization based approaches can achieve same/better guarantee much faster speed.
% 	\item First zero-th order result?
% \end{itemize}

% \textbf{Main application:}
% \begin{itemize}
% 	\item Empirical loss vs population loss, uniform convergence
% \end{itemize}

\input{related}


==> introduction_backup2.tex <==
% !TeX root = main.tex 

\section{Introduction}

Optimizing nonconvex loss functions has been the key to the success of modern machine learning. 
% This has strongly motivated gradient-based optimization algorithms for nonconvex functions. 
Unlike convex functions that usually have a unique critical point that is both locally and globally minimal, a nonconvex function can have many local maxima, local minima and saddle points, which pose significant challenges for optimization. A recent line of results \citep[e.g.,][]{ge2015escaping, carmon16accelerated,agarwal17finding,jin17escape} guarantees avoiding saddle points efficiently, hence resolving a family of matrix problems \cite[e.g.][]{bhoj16global, ge2016matrix} where all the local minima are desirable solutions. However, suboptimal local minima do exist in many important applications including Gaussian mixture \citep{jin2016local}, deep networks \citep{safran2017spurious}, etc.
and avoiding those undesirable local minima remains a challenging problem. %limited.

% While it is NP-hard to find global minima for a general nonconvex function, this paper shows how to efficiently avoid an important class of shallow local minima created by small perturbations to the ground truth function.
% %whose basins of attraction have ``low barriers'' 
% Suppose we are given a nonconvex function $f$ with a landscape that is problematic for optimization---possibly nonsmooth, with many `shallow' local minima---but we know that $f$ is close in function value to a well-behaved function $F$, which is smooth and do not have bad local minima, as shown in Figure \ref{fig:intro}a. Our objective is to find the `deep' local minima that persist in $F$, while avoiding those `shallow' local minima of $f$ that vanish in %the smoothed version %we shouldn't call F the smoothed version because later there is also f_\sigma and it can be confusing
% $F$.

While it is NP-hard to find global minima for a general nonconvex function, this paper shows how to efficiently avoid an important class of shallow local minima created by small perturbations to the objective function. In many learning scenarios, there exists an ground-truth function $F$ we would like to optimize, which is typically smooth. However, we are only given access to an erroneous function $f$ which is possibly non-smooth, even with many shallow local minima as shown in Figure \ref{fig:intro}a.
The only connection between $f$ and $F$ is that they are pointwise-close by error $\nu$:
\begin{equation}\label{eq:problem_intro}
    \norm{F - f}_{\infty} \le \nu. 
\end{equation}
Our objective is to find the approximate local minima (see definition \ref{def:exactSOSP}) of smooth function $F$, and avoid those shallow minima that only exist in erroneous $f$ but vanishe in ground-truth $F$.

% Suppose we are given a nonconvex function $f$ with a landscape that is problematic for optimization---possibly nonsmooth, with many `shallow' local minima---but we know that $f$ is close in function value to a well-behaved function $F$, which is smooth and do not have bad local minima, as shown in Figure \ref{fig:intro}a. Our objective is to find the `deep' local minima that persist in $F$, while avoiding those `shallow' local minima of $f$ that vanish in %the smoothed version %we shouldn't call F the smoothed version because later there is also f_\sigma and it can be confusing
% $F$. Formally, we assume the existence of smooth function $F$ which is point-wise close to the observed function $f$ by error $\nu$: 
% \begin{equation}\label{eq:problem_intro}
%     \norm{F - f}_{\infty} \le \nu. 
% \end{equation}
% The goal is to find the approximate local minima (see definition \ref{def:exactSOSP}) of function $F$ given only the function values of $f$.
% %\cnote{It's better if we can point out in the paper which are sharp shallow local minima, and which are flat deep local minima.}

This problem naturally arises in the context of \textit{empirical risk minimization (ERM)}, where $(f, F)$ are the empirical and population risks.
Given a nonconvex loss function $L(\btheta; \z)$ and data $\z_i$ sampled from an underlying distribution $\D$, the population risk $F(\btheta) = \E_{\z \sim \D}[L(\btheta; \z)]$ is the expectation of the loss function over the distribution $\D$; the empirical risk $f(\btheta) = \sum_{i=1}^n L(\btheta; \z_i)/n$ is the average of loss function over $n$ samples. While 
Population risk is always of primary interest in machine learning, learning algorithms only have access to empirical risk. The pointwise closeness between the two is typically guaranteed by by uniform convergence results from classical empirical process theory \citep{boucheron,bartlett03rademacher}. It is observed in deep learning that the empirical risk can have a landscape that is problematic for optimization, including exponentially many shallow local minima, even when the underlying population risk is well-behaved and smooth almost everywhere. \citep{brutzkus17globally,auer96exponentially}, as illustrated in Figure \ref{fig:intro}b.


% The empirical risk is often known to have a landscape that is problematic for optimization, even when the underlying population risk is well-behaved, as illustrated in Figure \ref{fig:intro} b. For example,
% the empirical risk can be nonsmooth in an entire subspace while the population 
% risk is smooth except at a single point (e.g., for convolution networks with 
% Gaussian inputs \citep{brutzkus17globally}). Sampling can introduce 
% exponentially many local minima \citep{auer96exponentially}. 
% In the context of deep learning, many researchers turn to studying the 
% population risk \citep{brutzkus17globally, li2017convergence} while analysis
% of its finite-sample version remains elusive, making it difficult to rule out the existence of local minima. %Even in low-rank matrix problems where analysis of the population risk is straightforward, the analysis of the empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}. 
% This motivates optimization algorithms that are immune to `shallow' local minima.




% In some applications \cite[e.g.][]{bhoj16global, ge2016matrix}, all the local minima are desirable solutions, while saddle points are not acceptable. Recent results in nonconvex optimization \citep[e.g.,][]{ge2015escaping, carmon16accelerated,agarwal17finding,jin17escape} guarantee avoiding saddle points when the objective function is smooth.  In contrast, our understanding of undesirable local minima is very limited. Although such local minima have suboptimal loss, the aforementioned guarantees do not preclude convergence to such minima.
% % in practical learning problems, one often encounters functions that are nonsmooth and have undesirable local minima, in which case these guarantees are no longer applicable.
% %Two key obstables to this are saddle points and local minima with suboptimal loss. 

% Since one cannot hope to deal with arbitrarily bad local minima, this paper is concerned with resolving an important class of spurious local minima that arises naturally in nonconvex \textit{empirical risk minimization}. Suppose we want to minimize a nonconvex function $f$, which may have a landscape that is problematic for optimization--- nonsmooth, with many poor local minima. Further, suppose it is known that $f$ is close in function value to $F$, which is also nonconvex but smooth and has no poor local minima, even though their higher order derivatives may be far apart (see Figure \ref{fig:intro}a):
% \begin{equation*}
% 	\norm{F - f}_{\infty} \le \nu. 
% \end{equation*}
% We do not have access to $F$, but would like to use this property to avoid poor local minima in $f$. Specifically, we want to converge to a ``flat'' local minimum of $f$---one that is close to being a local minimum in the smooth function $F$---as opposed to a ``sharp'' local minimum of $f$, that is, one that is far from being a local minimum in $F$.

% Let us consider the motivating application, empirical risk minimization.  
% Given a nonconvex loss function $L(\btheta; \z)$ and data $\z_i$ sampled from 
% an underlying distribution $\D$, the population risk $\poploss$ and empirical 
% risk $\emploss$ are $	\poploss(\btheta) = \E_{\z \sim \D}[L(\btheta; \z)]$ and $ \emploss(\btheta) = \frac{1}{n}\sum_{i=1}^n L(\btheta; \z_i)$ respectively. Learning algorithms only have access to the empirical risk---the average loss over training examples. Yet the empirical risk is often known to have a landscape that is problematic for optimization, even when 
% the underlying population risk is well-behaved, as illustrated in Figure \ref{fig:intro}.  Indeed,
% the empirical risk can be nonsmooth in an entire subspace while the population 
% risk is smooth except at a single point (e.g., for convolution networks with 
% Gaussian inputs \citep{brutzkus17globally}), and sampling can introduce 
% exponentially many spurious local minima \citep{auer96exponentially}. 
% In the context of deep learning, many researchers turn to studying the 
% population risk \citep{brutzkus17globally, li2017convergence} while analysis
% of its finite-sample version remains elusive, making it difficult to rule out the existence of poor local minima. Even in low-rank matrix problems 
% where analysis of the population risk is straightforward, the analysis of the 
% empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}. 


%\cnote{Put empirical risk after formulation, shorten current two paragraph, suffice to argue why our formulation is natual and interesting.}


\begin{figure}[t]
	\centering
	\includegraphics[width=0.28\textwidth, trim=80 70 250 10, clip]{nu_example.pdf}%
	\includegraphics[width=0.36\textwidth, trim=0 30 30 10, clip]{intro_pop}%
	\includegraphics[width=0.36\textwidth, trim=0 30 30 10, clip]{intro_emp}
	\caption{a) Function error $\nu$; b) Population risk vs empirical risk} \label{fig:intro}
\end{figure}
%\cnote{make f and F color in Figure 1 more distinguishable?}

% Fortunately, the empirical risk is typically pointwise close to the population risk and in some cases, one can show that the population risk is smooth and has no spurious local minima  \citep{brutzkus17globally, li2017convergence}. Using our formulation from earlier, $(F, f)$ might be the population and 
% empirical risk, $(\poploss, \emploss)$.  The function error $\nu$ may 
% be bounded by uniform convergence results from classical empirical process 
% theory \citep{boucheron,bartlett03rademacher}; it is typically 
% of order $O(1/\sqrt{n})$, closely related to the number of samples $n$. The size of $\nu$ also determines the degree of tolerance of poor local minima in $f$; intuitively, from Figure \ref{fig:intro}a, one can see that the smaller $\nu$ is, the `shallower' the spurious local minima in $f$ has to be.

%Fortunately, the empirical risk is often close in function value to another function that has a good landscape for optimization, even though their higher order derivatives may be far apart. For example, the empirical risk is typically pointwise close to the population risk and in some cases, one can show that the population risk is smooth and has no spurious local minima  \citep{brutzkus17globally, li2017convergence}. This implies that any local minima present in the empirical risk must be relatively `shallow', depending on how far it is from a well-behaved target function. Can we escape such local minima? This motivates the central problem in this paper, formally stated as follows.
%
%In the statistical learning setting, 
%
%\cnote{Put this formulation in second paragraph, and say our objective is that if our given function $F$is close to some smooth function $f$, we want to escape those ``sharp'' local minima, and find those local minima persist in the smooth function.}

The key quantity in problem \eqref{eq:problem_intro} is how much error $\nu$ we can tolerate. An algorithm that can tolerate larger $\nu$ also  escapes `deeper' local minima.  In the context of ERM, this means we require fewer samples to have the same guarantee on avoiding local minima.
To escape shallow local minima in the form of Problem \eqref{eq:problem_intro}, most previous work are based on ideas related sampling %Most previous work on Problem \eqref{eq:problem_intro} resort to significant noise to escape local minima,  under sampling-based algorithms 
such as simulated annealing \citep{belloni2015escaping}, or stochastic gradient Langevin dynamics (SGLD) \citep{zhang2017hitting}. %Such algorithms asymptotically converge to stationary distributions instead of the vicinity around local optima. Moreover, 
%I'm not sure if we should mention this as our algorithm also asymptotically converge to stationary distributions because we fix a step size. We can of course decrease our step size slowly but the sampling algorithms can also lower the temperature slowly.
These techniques require the algorithm to add a significant amount of noise in the optimization procedure. Such extra noise could hurt the convergence of the algorithms and does not allow them to escape deeper local minima: 
the only existing work that does not assume $F$ to be convex \citep{zhang2017hitting}, requires error $\nu$ to smaller than $O(\epsilon^2/d^8)$ where $\epsilon$ is the precision of the optimization guarantee (see Definition \ref{def:exactSOSP}) and $d$ is the problem dimension (see Figure~\ref{fig:contri}). 
% Most existing work has tackled this problem in the setting where $F$ is 
% convex \citep{belloni2015escaping,singer15information,risteski16alg}. 
% \citet{zhang2017hitting} showed how to solve the nonconvex version of 
% the problem using a sampling-based algorithm with suboptimal guarantees. Specifically, their algorithm requires $\nu$ to be have the order $\epsilon^2/d^8$ where $\epsilon$ is the precision of the optimization guarantee (see Definition \ref{def:exactSOSP}) and $d$ is the problem dimension (see Figure~\ref{fig:contri}). Hence the algorithm can only escape extremely `shallow' local minima in $f$. In addition, the sampling-based algorithm adds Gaussian noise to the iterates, and converges asymptotically to a stationary distribution. In contrast, an algorithm based on stochastic gradient descent only adds a small amount of perturbation and asymptotically converges to a neighborhood around the local minimum. 
%\cnote{Talk about deep first then Yuchen's work}


We would thus like to answer the two central questions: \textbf{ 1) Can a simple, optimization-based algorithm also avoid shallow local minima?
2) Can we tolerate larger error $\nu$, thus escaping `deeper' local minima? What is the largest error that the best algorithm can tolerate?} 

%Thus we would like to find the dependency of the quality of 
%the solution on  $\nu$. This raises the following central question:
%
%\textbf{How much error $\nu$ can we tolerate to (1) identify the approximate 
%	local minima (see Definition \ref{def:exactSOSP}) of $F$; and (2) efficiently 
%	find the approximate local minima of $F$? } Also, in the latter scenario, can a 
%simple algorithm such as stochastic gradient descent (SGD) achieve this goal?
 % on this approach. 
% study this optimization problem assuming target function $F$ is convex;
%the only work \citep{zhang2017hitting} that can solve this optimization problem in the nonconvex setting relies on a sampling-based method known as Stochastic Gradient Langevin Dynamics (SGLD) \citep{welling11bayesian}. To get an $\epsilon$-approximate solution (see Definition~\ref{def:SOSP}), \citet{zhang2017hitting} can only tolerate a very small function error $\nu = O(\epsilon^2/d^8)$
%\footnote{We note the difference between $\nu$ claimed here and $\nu = O(\epsilon^2)$ claimed in \citep{zhang2017hitting} is due to difference in assumptions. This paper assume Hessian Lipschitz with respect to the standard spectral norm; \citet{zhang2017hitting} assume it with respect to nuclear norm, with their Hessian Lipschitz constant naturally depends on dimension $d$.} with many technical assumptions tailored for sampleing-based algorithms.

%\cnote{Change up to here.}

In this paper, we provide affirmative answer to both questions, and establish optimal dependencies between the error $\nu$ and the precision of a solution~$\epsilon$. 
We propose a simple algorithm based on 
SGD (Algorithm~\ref{algo:PSGD}) which is guaranteed to find approximate 
local minima of $F$ efficiently if $\nu \le O(\epsilon^{1.5}/d)$, 
thus escaping all saddle points of $F$ and all the additional local minima 
introduced by $f$. Moreover, we provide a matching lower bound (up to logarithmic factors) for all algorithms making a polynomial number of queries of $f$.
% showing whenever $\nu \ge \tilde{\Omega}(\epsilon^{1.5}/d)$, no algorithm can successfully achieve above objective within polynomial number of queries to $f$ in the worst case, 
The lower bound shows that our algorithm achieves the optimal trade-off between $\nu$ and $\epsilon$, as well as the optimal dependence on problem dimension $d$.
%, among all algorithms making a 
%polynomial number of queries.
% give a simple optimization algorithm based on SGD (Algorithm~\ref{algo:PSGD}) that can achieve the optimal trade-off between $\nu$ and $\epsilon$, as well as the optimal dependence on problem dimension $d$, among all algorithms making polynomial number of queries. 
We also consider an information-theoretic limit to identify a approximate local 
minimum of $F$ regardless of the polynomial number of queries. We give a sharp information-theoretic 
threshold $\nu = \Theta(\epsilon^{1.5})$ (see Figure~\ref{fig:contri}). 

As a concrete example of the application to minimizing population risk, we show 
that our results can be directly used to give sample complexities for learning 
a ReLU unit, whose empirical risk is nonsmooth while population risk is smooth almost everywhere.  We note that other applications of our framework include two-stage robust 
optimization and private learning (see Section \ref{sec:otherapplications}). 
In these settings, $\nu$ can be viewed as the amount of adversarial perturbation 
or noise due to sources other than data sampling.
%
%
%The standard approach to controlling the effect of the differences between these
%risks requires a combination of statistical guarantees and algorithmic guarantees 
%from optimization: the former focuses on the connection between population risk 
%and empirical risk, and in particular the connection between the empirical risk 
%minimizer (ERM) and the population risk minimizer, while 
%the latter focuses on the empirical risk and tries to guarantee that an ERM
%can be found. Such analyses are much less straightforward in the nonconvex 
%setting notably because empirical risk minimization is not guaranteed when the 
%loss $L$ is nonconvex. Indeed, recent results in nonconvex 
%optimization \citep[e.g.,][]{ge2015escaping, carmon16accelerated,agarwal17finding,jin17escape} generally require that the objective function is smooth and has no spurious 
%local minima. These properties tend to hold only for the population risk, but 
%not for the empirical risk.%In many settings these algorithms cannot be directly applied to obtain ERM as empirical risk can be nonsmooth and have spurious local minima. 
%
%
%The landscape of empirical risk for nonconvex losses can be rough even when 
%the underlying population risk is smooth, as illustrated in Figure \ref{fig:intro}.  Indeed,
%the empirical risk can be nonsmooth in an entire subspace while the population 
%risk is smooth except at a single point (e.g., for convolution networks with 
%Gaussian inputs \citep{brutzkus17globally}), and sampling can introduce 
%exponentially many spurious local minima \citep{auer96exponentially}. 
%In the context of deep learning, many researchers turn to studying the 
%population risk \citep{brutzkus17globally, li2017convergence} while analysis
%of its finite-sample version remains elusive. Even in low-rank matrix problems 
%where analysis of the population risk is straightforward, the analysis of the 
%empirical risk can be highly non-trivial \citep{bhoj16global, ge2016matrix, ge2017no}. 
%
%Our goal in this paper is to show how to design algorithms that, despite 
%only having access to the rough empirical risk, can still optimize the population 
%risk efficiently. Our approach guarantees convergence in population risk with 
%minimal assumptions on its regularity, thus helping to bridge the gap between 
%statistics and nonconvex optimization. 
%As long as the population risk has a well-behaved landscape and is close to the empirical risk in function value, 
%In order to achieve our goal, we design algorithms that are robust to  the differences between population and empirical risk, so that nice population risk can already guarantee the success of optimization algorithm despite the possible bad landscape of empirical loss. 


%
%Nonconvex optimization has become a core topic in modern machine learning. It has wide applications including deep neural networks, reinforcement learning, matrix/tensor factorizations and Bayesian inference. %Traditional nonconvex optimization focus on finding stationary points which can be local minima, local maxima, or even saddle points []. While recent line of works
%Understanding the convergence rates and properties for nonconvex optimization algorithms received a lot of recent attention. In particular, a line of work  \citep{jin17escape, ge2015escaping} showed how to deal with saddle points and converge to local minima efficiently. Getting to a local minimum is also shown to be sufficient for many practical problems \cite{}.
%
%All the nonconvex optimization algorithms mentioned before require access to accurate estimates of function value and its gradient. However, in many statistical applications, the gradient information may not be available, and even the function value can be hard/costly to estimate. In this paper we focus on a {\em robust optimization} problem: 
%Here $\nu$ can be viewed as amount of adversarial perturbation or a measure of uncertainty over the function values of $F$. Given access to $f$, the goal is to find a point that is an approximate local minimum of $F$. %This setting 
%while $F$ is assumed to be smooth, $f$ can be highly-nonsmooth and introduing many additional shallow local minima (see Figure \ref{fig:intro}). Quantitaty $\nu$ can be viewed as adversarial perturbation to true function $F$. The objective of this paper is to find the second-order stationary point (also called approximate local minima) of $F$ satisfying $\grad F(\x) = 0$ and $\hess F(\x) \succeq 0$, thus escaping all the shallow local minima introduced by $f$.


%This general problem has many applications. For example, consider a statistical learning problem with a nonconvex loss function $L_w(x,y)$ for each sample $(x,y)\sim \D$. What we really want to optimize is the population loss $F(w) = \E_{(x,y)\sim \D}[L_w(x,y)]$. However, what we have access to is the empirical loss, which is just the average over the training examples. For many choices of $L$ (e.g. a 0/1 classification loss) even though $F$ can be well-behaved, $f$ is highly non-smooth and we can only guarantee the point-wise closeness of the two functions (see Figure~\ref{fig:intro}). In this setting the uncertainty $\nu$ is closely related to the number of samples, and we would like to get tight dependencies between $\nu$ and the quality of solution. % where $F$ is the population loss, typically nice-behaved due to its averaging nature; $f$ is the empirical loss, typically highly non-smooth and can introduce many additional shallow local minima. The point-wise closeness of $(F, f)$ is guaranteed by standard uniform convergence results []. 


%
%
%The central questions in this problem are \textbf{how much perturbation $\nu$ can we tolerate to 1) identify the SOSP of $F$; 2) efficiently find the SOSP of $F$? and in latter scenario, can simple algorithm such as SGD achieve this goal?}
%
%There has been many researches under this general framework in recent years (e.g. \citep{belloni2015escaping,singer15information,risteski16alg}), however, this line of works has been focused on the special case where underlying function $F$ is convex, and the objective is to find the global optimal of $F$. For general nonconvex $F$, \citet{zhang2017hitting} proposed a sampling based algorithm---stochastic gradient Langevin dynamics (SGLD), and proved that algorithm will succeed if perturbation is small $\nu \le O(\epsilon^{2}/d^8)$. It remains unclear if this small perturbation level is necessary to guarantee escaping shallow local minima.
%
%In this work, we proposed a simple optimization based algorithm --- zero-th order stochastic gradient descent, showing if finds the SOSP of $F$ and thus escaping all shallow local minima of $f$ given perturbation $\nu \le O(\epsilon^{1.5}/d)$, allowing significant more perturbation compared to previous work. On the other hand, we also proved while it is information-theoretical impossible to identify the SOSP of $F$ if $\nu \ge \Omega(\epsilon^{1.5})$, no polynomial algorithm can find the SOSP of $F$ if
%$\nu \ge \tilde{\Omega}(\epsilon^{1.5}/d)$ matching the noise tolerance of our SGD algorithm up to logarithmic factors.

%\cnote{Maybe use real line axis, think about exponential learnable or not learnable}
%\cnote{Say something about the techniques and examples}
%\cnote{Say difference between Langevin and our algorithm}
%
%\lnote{Notes from meeting with Mike (Feb 13). There has been a lot of progress in convex and nonconvex optimization, but not enough attention has been paid to the interplay between statistics and optimization. In particular, gradient based methods often assume that the objective function being optimized is well-behaved (smooth, no local minima) when oracles only have access to a less well-behaved \emph{approximation} to the true objective. This may be due to sampling, privacy or  nested objectives (e.g. in robust optimization formulations). Stochasticity in optimization introduces a problem where the exact objective is not known. The approximate objective function may have a rough surface with a drastically different differential landscape, so the guarantees of many sophisticated gradient and Hessian-based optimization methods no longer hold in this setting. Moreover, sampling can introduce shallow local minima. Our work takes a step towards bridging this gap between optimization theory and statistics.}


\begin{figure}[t]
\centering
\includegraphics[width=.9\textwidth]{contribution3.png}
\caption{Complete characterization of error $\nu$ vs accuracy $\epsilon$ and dimension $d$.} \label{fig:contri}
\end{figure}

% What is the completeness characterization of $\nu$ vs the hardness?
% Is gradient Langevin (or sampling based algorithm) necessary to solve this problem?








% \textbf{Conjecture:}
% \begin{itemize}
% 	\item Given zero-th order oracle $f(\x)$ so that $\sup_{\x}|f(\x) - F(\x)| \le \poly(\epsilon, \frac{1}{d})$, 
% 	where $F$ is $\ell$-gradient Lipschitz and $\rho$-Hessian Lipschitz. Then, stochastic gradient with perturbation will find second-order stationary point of $F$ in $\poly(\epsilon, d)$ iterations.
% \end{itemize}


% % \item Given first order oracle $\g(\x)$ so that $\sup_{\x} \norm{\g(\x) - \grad F(\x)} \le \poly(\epsilon, \frac{1}{d})$,
% % perturbed gradient descent (with $\g(\x)$) will find second order stationary point of $F$ with sharper rate.


% \textbf{Goal:}
% \begin{itemize}
% 	\item Finding second-order stationary with zero-th order oracle (rate).
% 	\item Finding second-order stationary with zero-th order oracle of point-wise close function (rate).
% 	Describe what are the additional local minima, and how smoothing technique removes them. 
% 	\item Connection to \citep{belloni2015escaping,zhang2017hitting,mei2016landscape,loh2013regularized}
% 	\begin{itemize}
% 		\item \citet{belloni2015escaping}: Assume F is (strongly) convex. Compare their result to our smoothing + SGD strategy, in terms of the $d$ and $\epsilon$ dependence in the iteration complexity and $\nu$.
% 		\item \citet{mei2016landscape}: Assume $f$ (or equivalently the loss function in statistical learning) is differentiable. They have results for gradient and Hessian difference without smoothing.
% 	\end{itemize}
% \end{itemize}

% \textbf{Contribution:}
% \begin{itemize}
% 	\item Removing a lot of redundant assumptions. State better results in a cleaner way.
% 	\item Show given this closeness to a good function (application in statistical setting), sampling based algorithm is not necessary for escaping shallow local minima. Optimization based approaches can achieve same/better guarantee much faster speed.
% 	\item First zero-th order result?
% \end{itemize}

% \textbf{Main application:}
% \begin{itemize}
% 	\item Empirical loss vs population loss, uniform convergence
% \end{itemize}

\input{related}

